Cross-correlation Weak Lensing of SDSS Galaxy Clusters III: Mass-to-light Ratios

We present measurements of the excess mass-to-light ratio measured aroundMaxBCG galaxy clusters observed in the SDSS. This red sequence cluster sample includes objects from small groups with masses ranging from ~5x10^{12} to ~10^{15} M_{sun}/h. Using cross-correlation weak lensing, we measure the excess mass density profile above the universal mean \Delta \rho(r) = \rho(r) - \bar{\rho} for clusters in bins of richness and optical luminosity. We also measure the excess luminosity density \Delta l(r) = l(r) - \bar{l} measured in the z=0.25 i-band. For both mass and light, we de-project the profiles to produce 3D mass and light profiles over scales from 25 kpc/ to 22 Mpc/h. From these profiles we calculate the cumulative excess mass M(r) and excess light L(r) as a function of separation from the BCG. On small scales, where \rho(r) >> \bar{\rho}, the integrated mass-to-light profile may be interpreted as the cluster mass-to-light ratio. We find the M/L_{200}, the mass-to-light ratio within r_{200}, scales with cluster mass as a power law with index 0.33+/-0.02. On large scales, where \rho(r) ~ \bar{\rho}, the M/L approaches an asymptotic value independent of cluster richness. For small groups, the mean M/L_{200} is much smaller than the asymptotic value, while for large clusters it is consistent with the asymptotic value. This asymptotic value should be proportional to the mean mass-to-light ratio of the universe <M/L>. We find <M/L>/b^2_{ml} = 362+/-54 h (statistical). There is additional uncertainty in the overall calibration at the ~10% level. The parameter b_{ml} is primarily a function of the bias of the L <~ L_* galaxies used as light tracers, and should be of order unity. Multiplying by the luminosity density in the same bandpass we find \Omega_m/b^2_{ml} = 0.02+/-0.03, independent of the Hubble parameter.

==> Makefile <==
TEXFILE=maxbcg_m2l
default: dvi

# just run it
bib: 
	bibtex ${TEXFILE}

dvi: 
	latex ${TEXFILE}
	latex ${TEXFILE}

ps: 
	dvips -t letter ${TEXFILE} -o ${TEXFILE}.ps

pdf:
	latex ${TEXFILE}
	latex ${TEXFILE}
	dvipdfm ${TEXFILE}.dvi #${TEXFILE}.pdf

# Remember to go ahead and make inside the astro-ph directory because
# they don't run bibtex
dir=${TEXFILE}_astro_ph
aph:
	rm -rf ${dir}
	rm -f ${dir}.tar.gz
	mkdir ${dir}
	mkdir ${dir}/plots
	cp maxbcg_m2l.bbl ${dir}/
	cp *.tex ${dir}/
	cp *.cls ${dir}/
	cp plots/*.eps ${dir}/plots/
	cp Makefile ${dir}/
tar:
	rm -f ${dir}.tar.gz
	tar cvfz ${dir}.tar.gz ${dir}



clean:
	rm \
	${TEXFILE}.dvi \
	${TEXFILE}.ps \
	${TEXFILE}.pdf \
	${TEXFILE}.aux \
	${TEXFILE}.bbl \
	${TEXFILE}.blg \
	${TEXFILE}.log 




